CLARA: Clarification of Language Ambiguity through Result Analysis for Natural-Language Cancer Genomics Queries

A natural language interface can be used to make cancer genomics databases easier to use, but even if a question is perfectly fluent, its scientific meaning can be ambiguous. We propose CLARA, a framework that represents a question as a typed scientific query specification, considers a few possible interpretations, executes them, and asks for clarification when the estimates diverge. CLARA was assessed on mutation-prevalence contrasts among eight TCGA PanCancer Atlas cohorts and a 30-gene panel. This benchmark consisted of 330 unique executable contrasts varying in mutation scope, assay denominator, and sample context; 115 contrasts were result-sensitive and 215 were result-stable, per the preregistered definition of relative divergence greater than 0.10 or absolute divergence greater than 5 percentage points. An independently implemented pandas execution engine perfectly replicated all 660 results from the SQLite engine. In a separate 120-question LLM-generated, manually vetted language stress test, CLARA recognized all 60 result-sensitive contrasts and needlessly clarified 13 of 60 stable contrasts (accuracy 89.2%, sensitivity/recall 100%, specificity 78.3%). Standalone machine learning had superior overall accuracy (97.5%) but missed one critical contrast. This demonstrates that downstream execution can distinguish consequential from inconsequential ambiguity and reveal an explicit trade-off between safety and burden.

==> cover_letter.tex <==
\begingroup
\setlength{\parindent}{0pt}
\setlength{\parskip}{0.65em}

COVER LETTER

July 27, 2026

Pacific Symposium on Biocomputing 2027 Program Committee

Re: CLARA: Clarification of Language Ambiguity through Result Analysis for Natural-Language Cancer Genomics Queries

Corresponding author email: pratyushs2009@gmail.com

Requested PSB session: Precision Medicine: Computational and AI Approaches for Understanding the Biological Basis of Health and Disease

Dear PSB 2027 Program Committee,

Please consider the enclosed manuscript, “CLARA: Clarification of Language Ambiguity through Result Analysis for Natural-Language Cancer Genomics Queries,” for review in the session “Precision Medicine: Computational and AI Approaches for Understanding the Biological Basis of Health and Disease.”

The submitted paper contains original, unpublished results and is not currently under consideration elsewhere. All co-authors concur with the contents of the paper and approve its submission to PSB 2027.

LLM disclosure: Large language models were used to generate natural-language questions for a blinded language stress-test benchmark from constrained assignments that did not expose result-sensitivity labels, prevalence values, or parser rules; two project members manually screened the resulting questions. The authors reviewed, revised, and take full responsibility for the scientific content, analyses, citations, interpretations, and conclusions. No LLM was used to alter the frozen data, thresholds, statistical analyses, or reported results after evaluation.


\noindent
Sincerely,

\medskip

\noindent
Pratyush Shukla\\
Wakeland High School\\
Corresponding author\\
pratyushs2009@gmail.com

\endgroup
